CokeBERT: Contextual Knowledge Selection and Embedding towards Enhanced Pre-Trained Language Models

Several recent efforts have been devoted to enhancing pre-trained language models (PLMs) by utilizing extra heterogeneous knowledge in knowledge graphs (KGs) and achieved consistent improvements on various knowledge-driven NLP tasks. However, most of these knowledge-enhanced PLMs embed static sub-graphs of KGs ("knowledge context"), regardless of that the knowledge required by PLMs may change dynamically according to specific text ("textual context"). In this paper, we propose a novel framework named Coke to dynamically select contextual knowledge and embed knowledge context according to textual context for PLMs, which can avoid the effect of redundant and ambiguous knowledge in KGs that cannot match the input text. Our experimental results show that Coke outperforms various baselines on typical knowledge-driven NLP tasks, indicating the effectiveness of utilizing dynamic knowledge context for language understanding. Besides the performance improvements, the dynamically selected knowledge in Coke can describe the semantics of text-related knowledge in a more interpretable form than the conventional PLMs. Our source code and datasets will be available to provide more details for Coke.

==> back <==

\subsubsection{Transformer-based PLM}
% BERT & GPT

Neural models can learn large amounts of language knowledge from language modeling. Since the language knowledge covers the demands of many downstream NLP tasks and provides powerful representations of words and sentences, some researchers found that knowledge can be transferred to other NLP tasks easily. The transferred models are called Pre-trained Language Models (PLMs).

Language modeling is the most basic and most important NLP task. It contains a variety of knowledge for language understanding, such as linguistic knowledge and factual knowledge. For example, the model needs to decide whether it should add an article before a noun. This requires linguistic knowledge about articles. Another example is the question of what is the following word after ``Trump is the president of''. The answer is "America", which requires factual knowledge. Since language modeling is very complex, the models can learn a lot from this task. 

On the other hand, language modeling only requires plain text without any human annotation. With this feature, the models can learn complex NLP abilities from a very large-scale corpus. Since deep learning needs large amounts of data and language modeling can make full use of all texts in the world, PLMs significantly benefit the development of NLP research.


Inspired by the success of the Transformer, GPT~\cite{radford2018improving} and BERT~\cite{devlin2018bert} began to adopt the Transformer as the backbone of the pre-trained language models. GPT and BERT are the most representative Transformer-based pre-trained language models (PLMs). Since they achieved state-of-the-art performance on various NLP tasks, nearly all PLMs after them are based on the Transformer. In this subsection, we will talk about GPT and BERT in more detail.

GPT is the first work to pre-train a PLM based on the Transformer. The training procedure of GPT~\cite{radford2018improving} contains two classic stages: generative pre-training and discriminative fine-tuning. 

In the pre-training stage, the input of the model is a large-scale unlabeled corpus denoted as $\mathcal{U} = \{u_1, u_2,...,u_n\}$. The pre-training stage aims to optimize a language model. The learning objective over the corpus is to maximize a conditional likelihood in a fixed-size window:
	\begin{equation}
		\mathcal{L}_1(\mathcal{U}) = \sum_i \log P(u_i|u_{i-k}, ..., u_{i-1}; \Theta),
	\end{equation}
	where $k$ represents the size of the window, the conditional likelihood $P$ is modeled by a neural network with parameters $\Theta$.
	
	For a supervised dataset $\chi$, the input is a sequence of words $s = (w_1, w_2,..,w_l)$ and the output is a label $y$.  The pre-training stage provides an advantageous start point of parameters that can be used to initialize subsequent supervised tasks. At this occasion, the objective is a discriminative task that maximizes the conditional possibility distribution: 
	\begin{equation}
		\mathcal{L}_2(\chi) = \sum_{(s,y)} \log P(y|w_1, \cdots, w_l),
	\end{equation}
	 where $P(y|w_1, \cdots,w_l)$ is modeled by a K-layer Transformer. After the input tokens pass through the pre-trained GPT, a hidden vector of the final layer $\mathbf{h}_l^K$ will be produced. To obtain the output distribution, we add a linear transformation layer, which has the same size as the number of labels:
	 \begin{equation}
	 	P(y|w_1, \cdots, w_m) = \operatorname{Softmax}(\mathbf{W}_y\mathbf{h}_l^K).
	 \end{equation}
	 
	The final training objective is combined with a language modeling $\mathcal{L}_1$ for better generalization:
	\begin{equation}
		\mathcal{L}(\chi) = \mathcal{L}_2(\chi) + \lambda * \mathcal{L}_1(\chi), 
	\end{equation}
	 where $\lambda$ is a weight hyper-parameter. 

	\begin{figure}[t!]%%图
		\centering  %插入的图片居中表示
		\includegraphics[width=\linewidth]{figs/fig_ch4_sentence/fig-ch4-bert}
		\caption{The pre-training and fine-tuning stages for BERT.} 
		\label{fig-bert}
	\end{figure}

BERT~\cite{devlin2018bert} is a milestone work in the field of PLM. BERT achieved significant empirical results on 17 different NLP tasks, including SQuAD (outperform human being), GLUE (7.7\% point absolute improvement), MultiNLI (4.6\% point absolute improvement), etc. Compared to GPT, BERT uses a bidirectional deep Transformer as the model backbone. As illustrated in Fig. \ref{fig-bert}, BERT contains pre-training and fine-tuning stages.

In the pre-training stage, two objectives are designed: \textit{masked language model (MLM)} and \textit{next sentence prediction (NSP)}. (1) For MLM, tokens are randomly masked with a special token ${\rm [MASK]}$. The training objective is to predict the masked tokens based on the contexts. Compared with the standard unidirectional conditional language model, which can only be trained in one direction, MLM aims to train a deep bidirectional representation model. This task is inspired by \textit{Cloze} \cite{taylor1953cloze}. (2) The objective of NSP is to capture relationships between sentences for some sentence-based downstream tasks such as natural language inference (NLI) and question answering (QA). In this task, a binary classifier is trained to predict whether the sentence is the next sentence for the current. This task effectively captures the deep relationship between sentences, exploring semantic information from a different level.

After pre-training, BERT can capture various language knowledge for downstream supervised tasks. By modifying inputs and outputs, BERT can be fine-tuned for any NLP tasks, which contain the applications with the input of single text or text pairs. The input consists of sentence ${\rm A}$ and sentence ${\rm B}$, which can represent: (1) sentence pairs in paraphrase, (2) hypothesis-premise pairs in entailment, (3) question-passage pairs in QA, and (4) text-$\emptyset$ for text classification task or sequence tagging. For the output, BERT can produce the token-level representation for each token, which is used to sequence tagging task or question answering. Besides, the special token $[CLS]$ in BERT is fed into the classification layer for sequence classification. 

\subsubsection{PLM Family}

Pre-trained language models have rapid progress after BERT. We summarize several important directions of PLMs and show some representative models and their relationship in Fig. \ref{plm-family}.

Here is a brief introduction of the PLMs after BERT. Firstly, there are some variants of BERT for better general language representation, such as RoBERTa~\cite{liu2019roberta} and XLNet~\cite{yang2019xlnet}. These models mainly focus on the improvement of pre-training tasks. Secondly, some people work on pre-trained generation models, such as MASS~\cite{song2019mass} and UniLM~\cite{dong2019unified}. These models achieve promising results on the generation tasks instead of the natural language understanding (NLU) tasks used by BERT. Thirdly, the sentence pair format of BERT inspired works on the cross-lingual and cross-modal fields. XLM~\cite{conneau2019cross}, ViLBERT~\cite{lu2019vilbert}, and VideoBERT~\cite{sun2019videobert} are the important works in this direction. Lastly, there are some works~\cite{zhang2019ernie,peters2019knowledge} that explore to incorporate external knowledge into PLMs since some low-frequency knowledge cannot be efficiently learned by PLMs.

	\begin{figure}[t!]%%图
		\centering  %插入的图片居中表示
		\includegraphics[width=\linewidth]{figs/fig_ch4_sentence/fig-ch4-PLMfamily}
		\caption{The Pre-trained Language Model Family.} 
		\label{plm-family}
	\end{figure}
	

